On Generalization Error Bounds of Noisy Gradient Methods for Non-Convex Learning

Generalization error (also known as the out-of-sample error) measures how well the hypothesis learned from training data generalizes to previously unseen data. Proving tight generalization error bounds is a central question in statistical learning theory. In this paper, we obtain generalization error bounds for learning general non-convex objectives, which has attracted significant attention in recent years. We develop a new framework, termed Bayes-Stability, for proving algorithm-dependent generalization error bounds. The new framework combines ideas from both the PAC-Bayesian theory and the notion of algorithmic stability. Applying the Bayes-Stability method, we obtain new data-dependent generalization bounds for stochastic gradient Langevin dynamics (SGLD) and several other noisy gradient methods (e.g., with momentum, mini-batch and acceleration, Entropy-SGD). Our result recovers (and is typically tighter than) a recent result in Mou et al. (2018) and improves upon the results in Pensia et al. (2018). Our experiments demonstrate that our data-dependent bounds can distinguish randomly labelled data from normal data, which provides an explanation to the intriguing phenomena observed in Zhang et al. (2017a). We also study the setting where the total loss is the sum of a bounded loss and an additional \ell_2 regularization term. We obtain new generalization bounds for the continuous Langevin dynamic in this setting by developing a new Log-Sobolev inequality for the parameter distribution at any time. Our new bounds are more desirable when the noisy level of the process is not small, and do not become vacuous even when T tends to infinity.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> mini-batch-proof.tex <==
Let $G$ be the set of all possible mini-batches. $G_n = \{B \in G: n \in B\}$ denotes the collection of mini-batches that contain $n$, while $\overline{G_n} = G \setminus G_n$.
Let $\diam(A) = \sup_{x, y\in A}\|x-y\|$ denote the diameter of set $A$.
\begin{lemma11}
Suppose that batch size $b \le n/2$. 
$\{\mu_B: B \in G\}$ and $\{\mu'_B: B \in G\}$ are two collections of points in $\R^d$
labeled by mini-batches of size $b$ that satisfy the following conditions 
for some constant $\beta \in [0, \sigma]$:
\begin{enumerate}
   \item $\left\|\mu_B - \mu'_B\right\| \leq \beta$ for $B \in G_n$ and $\mu_B = \mu'_B$ for $B \in \overline{G_{n}}$.
   \item $\diam(\{\mu_B: B\in G\}\cup\{\mu'_B: B\in G\}) \le \sigma$.
\end{enumerate} 

Let $p_{\mu,\sigma}$ denote the Gaussian distribution $\N(\mu, \frac{\sigma^2}{2}I_d)$. 
Let $P = \frac{1}{|G|}\sum_{B \in G}p_{\mu_B,\sigma}$ and 
$P' = \frac{1}{|G|}\sum_{B \in G}p_{\mu'_B,\sigma}$ be two 
mixture distributions over all mini-batches. Then, for some universal constant $C_0$,
  \[\KL(P,P') \leq \frac{C_0b^2\beta^2}{\sigma^2n^2}.\]
\end{lemma11}
\begin{Proof}{\bf of Lemma~\ref{lem:mini-batch}}
By Lemma~\ref{lem:kl-dtd-bound}, $\KL(P,P')$ is bounded by
\begin{align*}
    \ln 2\cdot\DTD{P}{P'}
&=   \ln 2\cdot\sum_{k = 0}^{+\infty} 2^k \cdot \TD{2^{-k} P + (1-2^{-k})P'}{P'}\\
&=   \ln 2\cdot\sum_{k = 0}^{+\infty} 2^{k}\cdot\int_{\R^d}\frac{4^{-k}(P(w) - P'(w))^2}{2^{-k}P(w) + (2-2^{-k})P'(w)}~\rmd w.
\end{align*}
The numerator of the above integrand is upper bounded by
\begin{equation}\label{minibatchLemProof1}
\begin{split}
  4^{-k}(P - P')^2 
  &= 4^{-k}\left(\frac{1}{|G|}\sum_{B\in G}(p_{\mu_B, \sigma} - p_{\mu'_B, \sigma})\right)^2\\
  &= \frac{4^{-k}|G_n|^2}{|G|^2}\left(\frac{1}{|G_n|}\sum_{B\in G_n}(p_{\mu_B, \sigma} - p_{\mu'_B, \sigma})\right)^2\\ 
  &\leq \frac{4^{-k}b^2}{n^2}\cdot\frac{1}{|G_n|}\sum_{B\in G_n}(p_{\mu_B, \sigma} - p_{\mu'_B, \sigma})^2,
\end{split}
\end{equation}
while the denominator can be lower bounded as follows:
\begin{align*}
2^{-k}P + (2-2^{-k})P'
&\ge \frac{2^{-k}}{|G|}\sum_{B\in \overline{G_n}}p_{\mu_B, \sigma} 
  + \frac{2-2^{-k}}{|G|}\sum_{B\in \overline{G_n}}p_{\mu'_B, \sigma}\\
&= \frac{2}{|G|}\sum_{B\in \overline{G_n}}p_{\mu_B, \sigma} \tag{$\mu_B = \mu'_B$ for $B \in \overline{G_n}$}\\
&=\frac{1}{|\overline{G_n}|} \cdot \frac{2(n-b)}{n} \sum_{B\in \overline{G_n}}p_{\mu_B, \sigma}\\
&\geq \frac{1}{|\overline{G_n}|} \sum_{B\in \overline{G_n}}p_{\mu_B, \sigma}, \tag{$b \le n/2$}\\
\end{align*}
which implies, by the convexity of $1/x$, that
\begin{equation}\label{minibatchLemProof2}
    \frac{1}{2^{-k}P + (2-2^{-k})P'}
\le \frac{1}{\frac{1}{|\overline{G_n}|} \sum_{B\in \overline{G_n}}p_{\mu_B, \sigma}}
\le \frac{1}{|\overline{G_n}|} \sum_{B\in \overline{G_n}} \frac{1}{p_{\mu_B, \sigma}}.
\end{equation}

Inequalities \eqref{minibatchLemProof1}~and~\eqref{minibatchLemProof2} together imply
\begin{equation}\label{minibatchLemProof3}
    \TD{2^{-k} P + (1-2^{-k})P'}{P'}
\le \frac{4^{-k}b^2}{n^2|\overline{G_n}||G_n|}\sum_{A\in \overline{G_n}}
       \sum_{B\in G_n}
        \int_{\R^d}{\frac{(p_{\mu_B, \sigma}(w) - p_{\mu'_B, \sigma}(w))^2}{p_{\mu_A, \sigma}(w)}}~\rmd w.
\end{equation}

Now we bound the right-hand side of \eqref{minibatchLemProof3} for fixed $A$ and $B$. By applying a translation and a rotation, we can assume without loss of generality that $\mu_A = 0$, and the last $d-2$ coordinates of $\mu_B$ and $\mu_B'$ are all zero. Note that the integral is unchanged when we project the space to the two-dimensional subspace corresponding to the first two coordinates. Thus, it suffices to prove a bound for $d = 2$. We rewrite \eqref{minibatchLemProof3} as
\begin{equation}
\label{minibatchLemProof10}
\Delta(2^{-k} P + (1-2^{-k})P',P') 
  \leq \frac{4^{-k}b^2}{n^2|\overline{G_n}||G_n|}
        \sum_{A\in \overline{G_n}}\sum_{B\in G_n}
        \frac{1}{\pi\sigma^2}\int_{\R^2}{\frac{\left(e^{-\left\|\frac{w-\mu_B}{\sigma}\right\|^2} - e^{-\left\|\frac{w-\mu'_B}{\sigma}\right\|^2}\right)^2}{e^{-\left\|\frac{w}{\sigma}\right\|^2}}}~\rmd w
\end{equation}

Let $r = \left\|\frac{w}{\sigma}\right\|$ and $\delta = \beta / \sigma$. Since $\left\|\mu_B - \mu_A\right\| \leq \sigma$, $\left\|\mu'_B - \mu_A\right\| \leq \sigma$, and $\left\|\mu_B - \mu'_B\right\| \leq \beta$, we have
    \[\left\|\frac{w - \mu_B}{\sigma}\right\|, \left\|\frac{w - \mu'_B}{\sigma}\right\| \in [r - 1, r + 1]\]
and
    \[\left\|\frac{w - \mu_B}{\sigma}\right\| - \left\|\frac{w - \mu'_B}{\sigma}\right\| \in [-\delta, \delta].\]
It follows that 
\begin{equation}
\label{minibatchLemProof7}
\begin{split}
\left(e^{-\left\|\frac{w-\mu_B}{\sigma}\right\|^2} - e^{-\left\|\frac{w-\mu'_B}{\sigma}\right\|^2}\right)^2
&\le \max_{r-1 \le y \le r + 1}\left(e^{-y^2} - e^{-(y+\delta)^2}\right)^2.
\end{split}
\end{equation}
Let $g(y) = e^{-y^2} - e^{-(y+\delta)^2}$. By taking derivative w.r.t $y$, we have $g'(y) = -2y e^{-y^2} + 2(y + \delta)e^{-(y+\delta)^2}$. For fixed $y > 1$, let $h(x) = -2ye^{-y^2} + 2(y + x)e^{-(y + x)^2}$. Note that $h(0) = 0$ and for $x \ge 0$,
\begin{align*}
h'(x) &= 2e^{-(y + x)^2} - 4(y + x)^2e^{-(y+x)^2}\\
&= [2 - 4(y + x)^2] e^{-(y+x)^2} < 0. \tag{$y > 1$}
\end{align*}
Thus, $g'(y) < 0$ for any $y > 1$, which further implies that for $r > 2$, 
\[
\max_{r-1\leq y \leq r + 1}\left(e^{-y^2} - e^{-(y+\delta)^2}\right)^2 = \left(e^{-(r-1)^2} - e^{-(r-1+\delta)^2}\right)^2.
\]
Let $I(\delta) = \int_{2}^{+\infty}\frac{\left(e^{-(r-1)^2} - e^{-(r-1+\delta)^2}\right)^2}{e^{-r^2}}2\pi r~\rmd r$. By Taylor's theorem, for some $\xi \in [0, \delta]$,
\[I(\delta) = I(0) + \frac{I'(0)}{1!} \delta + \frac{I''(\xi)}{2!}\delta^2.\]
Since $I(0) = 0$, $I'(0) = 0$ and 
\begin{equation*}
\begin{split}
  I''(\xi) &= \int_{2}^{+\infty}2\pi r e^{r^2}\left.\left[\left(e^{-(r-1)^2} - e^{-(r-1+\delta)^2}\right)^2\right]''\right|_{\delta = \xi}~\rmd r\\
  &= \int_{2}^{+\infty}2\pi r e^{r^2} \left(8e^{-2(r+\xi -1)^2}(r+\xi-1)^2\right)~\rmd r\\
  &- \int_{2}^{+\infty}2\pi r e^{r^2} \left(8e^{-(r+\xi-1)^2}\left(e^{-(r-1)^2} - e^{-(r+\xi-1)^2}\right)(r+\xi-1)^2\right)~\rmd r\\
  &+ \int_{2}^{+\infty}2\pi r e^{r^2} \left(4e^{-(r+\xi-1)^2}(e^{-(r-1)^2} - e^{-(r+\xi-1)^2})\right)~\rmd r\\
  &\leq \int_{2}^{+\infty}2\pi r e^{r^2} \cdot 8e^{-2(r-1)^2}(r-1)^2~\rmd r\\
  &+ \int_{2}^{+\infty}2\pi r e^{r^2} \cdot 4e^{-2(r-1)^2}~\rmd r\\
  &\leq 2430.9 + 422.1 = 2853,
\end{split}
\end{equation*}
we have
\begin{equation}
\label{minibatchLemProof5}
I(\delta) = \int_{2}^{+\infty}\frac{\left(e^{-(r-1)^2} - e^{-(r-1+\delta)^2}\right)^2}{e^{-r^2}} 2\pi r~\rmd r \leq \frac{2853}{2}\delta^2
\end{equation}

Now we turn to the case that $r \leq 2$. For fixed $y$, let $\phi(\delta) = (e^{-y^2} - e^{-(y+\delta)^2})^2$. By Taylor's theorem, we have
\[
\phi(\delta) = \phi(0) + \frac{\phi'(0)}{1!} \delta + \frac{\phi''(\xi)}{2!}\delta^2
\]
for some $\xi \in [0, \delta]$.
Since $\phi(0) = 0$, $\phi'(0) = 0$ and 
\begin{align*}
\phi''(\xi) &= -8e^{-(\xi + y)^2}(e^{-y^2} - e^{-(\xi + y)^2})(\xi + y)^2
+4 e^{-(\xi+y)^2}(e^{-y^2}-e^{-(\xi+y)^2})
+8 e^{-2(\xi+y)^2}(\xi +y)^2\\
&\le 4e^{-1}
+4
+4e^{-1}
\le 7,
\end{align*}
we have $\phi(\delta) \leq \frac{7}{2}\delta^2$, and it follows that
\begin{equation}
\label{minibatchLemProof4}
\int_{0}^{2} \frac{\max_{r-1\leq y \leq r + 1}\left(e^{-y^2} - e^{-(y+\delta)^2}\right)^2}{e^{-r^2}} \cdot 2\pi r~\rmd r
\leq \int_{0}^{2} \frac{7}{2}\delta^2e^{r^2}\cdot2\pi r~\rmd r \leq \frac{1179}{2}\delta^2
\end{equation}

Combining \eqref{minibatchLemProof7}, \eqref{minibatchLemProof5} and \eqref{minibatchLemProof4}, we have
\begin{equation*}
\begin{split}
\frac{1}{\sigma^2}\int_{\R^2}{\frac{\left(e^{-\left\|\frac{w-\mu_B}{\sigma}\right\|^2} - e^{-\left\|\frac{w-\mu'_B}{\sigma}\right\|^2}\right)^2}{e^{-\left\|\frac{w}{\sigma}\right\|^2}}}~\rmd w
&\leq \int_{0}^{2} \frac{\max_{r-1\leq y \leq r + 1}\left(e^{-y^2} - e^{-(y+\delta)^2}\right)^2}{e^{-r^2}} 2\pi r~\rmd r\\
&+ \int_{2}^{+\infty}\frac{\left(e^{-(r-1)^2} - e^{-(r-1+\delta)^2}\right)^2}{e^{-r^2}} 2\pi r~\rmd r\\
&\leq 2016\delta^2.
\end{split}
\end{equation*}
Plugging the above into~\eqref{minibatchLemProof10} gives
    \[\Delta(2^{-k} P + (1-2^{-k})P',P') \le \frac{4^{-k}b^2}{\pi n^2}\cdot 2016\delta^2.\]
We conclude that
\begin{align*}
\KL(P,P') &\le \ln 2\cdot\sum_{k = 0}^{+\infty} 2^{k}\cdot\Delta(2^{-k} P + (1-2^{-k})P',P')\\
&\le \frac{2016\cdot\ln 2}{\pi}\cdot\frac{b^2\delta^2}{n^2}\sum_{k = 0}^{+\infty}2^{-k}
\le 890\frac{b^2\beta^2}{\sigma^2n^2}.
\end{align*}
\end{Proof}

\iffalse
\begin{copylemma}{\bf\ref{lem:mini-batch-2d}}
    Suppose that $A, B, C$ are Gaussian distributions on $\R^2$ with means $\mu_A, \mu_B, \mu_C$ and covariance matrix $\frac{1}{2}I$, such that $\mu_A = 0$ and $\diam(\{\mu_A, \mu_B, \mu_C\}) \le 1$. Then,
    \[\int_{\R^2}\frac{(B(w) - C(w))^2}{A(w)}~\rmd w \le	27.\]
\end{copylemma}
\begin{Proof}{\bf of Lemma~\ref{lem:mini-batch-2d}}
	Let $w$ be a point in $\R^d$ with $\norm{w} = r$. By the assumption that $\mu_A = 0$ and $\diam(\{\mu_A, \mu_B, \mu_C\}) \le 1$, we have
	\[\norm{w - \mu_B}, \norm{w - \mu_C} \in \left[\max(r - 1, 0), r + 1\right].\]
	The term $\frac{(B(w) - C(w))^2}{A(w)}$ is then at most
	\[\frac{1}{2\pi}\cdot\frac{\left[e^{-\max(r-1, 0)^2} - e^{-(r+1)^2}\right]^2}{e^{-r^2}}.\]
	Thus, the integral is upper bounded by
	\[
		\int_{\R^2}\frac{(B(w) - C(w))^2}{A(w)}~\textrm{d}w
	\le	\frac{1}{2\pi}\int_{0}^{+\infty}\frac{\left[e^{-\max(r-1, 0)^2} - e^{-(r+1)^2}\right]^2}{e^{-r^2}}\cdot2\pi r~\textrm{d}r
	\le	27.
	\]
\end{Proof}
\fi
